Fermion Masses and Mixings and Dark Matter Constraints in a Model with Radiative Seesaw Mechanism

We formulate a predictive model of fermion masses and mixings based on a $\Delta(27)$ family symmetry. In the quark sector the model leads to the viable mixing inspired texture where the Cabibbo angle comes from the down quark sector and the other angles come from both up and down quark sectors. In the lepton sector the model generates a predictive structure for charged leptons and, after radiative seesaw, an effective neutrino mass matrix with only one real and one complex parameter. We carry out a detailed analysis of the predictions in the lepton sector, where the model is only viable for inverted neutrino mass hierarchy, predicting a strict correlation between $\theta_{23}$ and $\theta_{13}$. We show a benchmark point that leads to the best-fit values of $\theta_{12}$, $\theta_{13}$, predicting a specific $\sin^2\theta_{23} \simeq 0.51$ (within the $3 \sigma$ range), a leptonic CP-violating Dirac phase $\delta \simeq 281.6 ^\circ$ and for neutrinoless double-beta decay $m_{ee} \simeq 41.3$ meV. We turn then to an analysis of the dark matter candidates in the model, which are stabilized by an unbroken $\mathbb{Z}_2$ symmetry. We discuss the possibility of scalar dark matter, which can generate the observed abundance through the Higgs portal by the standard WIMP mechanism. An interesting possibility arises if the lightest heavy Majorana neutrino is the lightest $\mathbb{Z}_2$-odd particle. The model can produce a viable fermionic dark matter candidate, but only as a feebly interacting massive particle (FIMP), with the smallness of the coupling to the visible sector protected by a symmetry and directly related to the smallness of the light neutrino masses.

==> biblio.tex <==
%\cite{Ishimori:2010au}
\bibitem{Ishimori:2010au}
  H.~Ishimori, T.~Kobayashi, H.~Ohki, Y.~Shimizu, H.~Okada and M.~Tanimoto,
  %``Non-Abelian Discrete Symmetries in Particle Physics,''
  Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 183} (2010) 1
  doi:10.1143/PTPS.183.1
  [arXiv:1003.3552 [hep-th]].
  %%CITATION = doi:10.1143/PTPS.183.1;%%
  %507 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Altarelli:2010gt}
\bibitem{Altarelli:2010gt}
  G.~Altarelli and F.~Feruglio,
  %``Discrete Flavor Symmetries and Models of Neutrino Mixing,''
  Rev.\ Mod.\ Phys.\  {\bf 82} (2010) 2701
  doi:10.1103/RevModPhys.82.2701
  [arXiv:1002.0211 [hep-ph]].
  %%CITATION = doi:10.1103/RevModPhys.82.2701;%%
  %576 citations counted in INSPIRE as of 12 Mar 2018



%\cite{King:2013eh}
\bibitem{King:2013eh}
  S.~F.~King and C.~Luhn,
  %``Neutrino Mass and Mixing with Discrete Symmetry,''
  Rept.\ Prog.\ Phys.\  {\bf 76} (2013) 056201
  doi:10.1088/0034-4885/76/5/056201
  [arXiv:1301.1340 [hep-ph]].
  %%CITATION = doi:10.1088/0034-4885/76/5/056201;%%
  %399 citations counted in INSPIRE as of 12 Mar 2018



%\cite{King:2014nza}
\bibitem{King:2014nza}
  S.~F.~King, A.~Merle, S.~Morisi, Y.~Shimizu and M.~Tanimoto,
  %``Neutrino Mass and Mixing: from Theory to Experiment,''
  New J.\ Phys.\  {\bf 16} (2014) 045018
  doi:10.1088/1367-2630/16/4/045018
  [arXiv:1402.4271 [hep-ph]].
  %%CITATION = doi:10.1088/1367-2630/16/4/045018;%%
  %194 citations counted in INSPIRE as of 12 Mar 2018



%\cite{King:2017guk}
\bibitem{King:2017guk}
  S.~F.~King,
  %``Unified Models of Neutrinos, Flavour and CP Violation,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 94} (2017) 217
  doi:10.1016/j.ppnp.2017.01.003
  [arXiv:1701.04413 [hep-ph]].
  %%CITATION = doi:10.1016/j.ppnp.2017.01.003;%%
  %29 citations counted in INSPIRE as of 12 Mar 2018



%\cite{deMedeirosVarzielas:2006fc}
\bibitem{deMedeirosVarzielas:2006fc}
  I.~de Medeiros Varzielas, S.~F.~King and G.~G.~Ross,
  %``Neutrino tri-bi-maximal mixing from a non-Abelian discrete family symmetry,''
  Phys.\ Lett.\ B {\bf 648} (2007) 201
  doi:10.1016/j.physletb.2007.03.009
  [hep-ph/0607045].
  %%CITATION = doi:10.1016/j.physletb.2007.03.009;%%
  %233 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Ma:2006ip}
\bibitem{Ma:2006ip}
  E.~Ma,
  %``Neutrino Mass Matrix from Delta(27) Symmetry,''
  Mod.\ Phys.\ Lett.\ A {\bf 21} (2006) 1917
  doi:10.1142/S0217732306021190
  [hep-ph/0607056].
  %%CITATION = doi:10.1142/S0217732306021190;%%
  %112 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Ma:2007wu}
\bibitem{Ma:2007wu}
  E.~Ma,
  %``Near tribimaximal neutrino mixing with Delta(27) symmetry,''
  Phys.\ Lett.\ B {\bf 660} (2008) 505
  doi:10.1016/j.physletb.2007.12.060
  [arXiv:0709.0507 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2007.12.060;%%
  %96 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2012nn}
\bibitem{Varzielas:2012nn}
  I.~de Medeiros Varzielas, D.~Emmanuel-Costa and P.~Leser,
  %``Geometrical CP Violation from Non-Renormalisable Scalar Potentials,''
  Phys.\ Lett.\ B {\bf 716} (2012) 193
  doi:10.1016/j.physletb.2012.08.008
  [arXiv:1204.3633 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2012.08.008;%%
  %52 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bhattacharyya:2012pi}
\bibitem{Bhattacharyya:2012pi}
  G.~Bhattacharyya, I.~de Medeiros Varzielas and P.~Leser,
  %``A common origin of fermion mixing and geometrical CP violation, and its test through Higgs physics at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 241603
  doi:10.1103/PhysRevLett.109.241603
  [arXiv:1210.0545 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.109.241603;%%
  %65 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Ma:2013xqa}
\bibitem{Ma:2013xqa}
  E.~Ma,
  %``Neutrino Mixing and Geometric CP Violation with Delta(27) Symmetry,''
  Phys.\ Lett.\ B {\bf 723} (2013) 161
  doi:10.1016/j.physletb.2013.05.011
  [arXiv:1304.1603 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.05.011;%%
  %27 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Nishi:2013jqa}
\bibitem{Nishi:2013jqa}
  C.~C.~Nishi,
  %``Generalized $CP$ symmetries in $\Delta(27)$ flavor models,''
  Phys.\ Rev.\ D {\bf 88} (2013) no.3,  033010
  doi:10.1103/PhysRevD.88.033010
  [arXiv:1306.0877 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.033010;%%
  %44 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2013sla}
\bibitem{Varzielas:2013sla}
  I.~de Medeiros Varzielas and D.~Pidt,
  %``Towards realistic models of quark masses with geometrical CP violation,''
  J.\ Phys.\ G {\bf 41} (2014) 025004
  doi:10.1088/0954-3899/41/2/025004
  [arXiv:1307.0711 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/41/2/025004;%%
  %34 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Aranda:2013gga}
\bibitem{Aranda:2013gga}
  A.~Aranda, C.~Bonilla, S.~Morisi, E.~Peinado and J.~W.~F.~Valle,
  %``Dirac neutrinos from flavor symmetry,''
  Phys.\ Rev.\ D {\bf 89} (2014) no.3,  033001
  doi:10.1103/PhysRevD.89.033001
  [arXiv:1307.3553 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.033001;%%
  %35 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2013eta}
\bibitem{Varzielas:2013eta}
  I.~de Medeiros Varzielas and D.~Pidt,
  %``Geometrical CP violation with a complete fermion sector,''
  JHEP {\bf 1311} (2013) 206
  doi:10.1007/JHEP11(2013)206
  [arXiv:1307.6545 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2013)206;%%
  %22 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Ma:2014eka}
\bibitem{Ma:2014eka}
  E.~Ma and A.~Natale,
  %``Scotogenic $Z_2$ or $U(1)_D$ Model of Neutrino Mass with $\Delta(27)$ Symmetry,''
  Phys.\ Lett.\ B {\bf 734} (2014) 403
  doi:10.1016/j.physletb.2014.05.070
  [arXiv:1403.6772 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2014.05.070;%%
  %33 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Abbas:2014ewa}
\bibitem{Abbas:2014ewa}
  M.~Abbas and S.~Khalil,
  %``Fermion masses and mixing in $\Delta(27)$ flavour model,''
  Phys.\ Rev.\ D {\bf 91} (2015) no.5,  053003
  doi:10.1103/PhysRevD.91.053003
  [arXiv:1406.6716 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.91.053003;%%
  %9 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2015aua}
\bibitem{Varzielas:2015aua}
  I.~de Medeiros Varzielas,
  %``$\Delta(27)$ family symmetry and neutrino mixing,''
  JHEP {\bf 1508} (2015) 157
  doi:10.1007/JHEP08(2015)157
  [arXiv:1507.00338 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2015)157;%%
  %18 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Abbas:2015zna}
\bibitem{Abbas:2015zna}
  M.~Abbas, S.~Khalil, A.~Rashed and A.~Sil,
  %``Neutrino masses and deviation from tribimaximal mixing in Δ(27) model with inverse seesaw mechanism,''
  Phys.\ Rev.\ D {\bf 93} (2016) no.1,  013018
  doi:10.1103/PhysRevD.93.013018
  [arXiv:1508.03727 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.013018;%%
  %10 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Chen:2015jta}
\bibitem{Chen:2015jta}
  P.~Chen, G.~J.~Ding, A.~D.~Rojas, C.~A.~Vaquera-Araujo and J.~W.~F.~Valle,
  %``Warped flavor symmetry predictions for neutrino physics,''
  JHEP {\bf 1601} (2016) 007
  doi:10.1007/JHEP01(2016)007
  [arXiv:1509.06683 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2016)007;%%
  %31 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bjorkeroth:2015uou}
\bibitem{Bjorkeroth:2015uou}
  F.~Björkeroth, F.~J.~de Anda, I.~de Medeiros Varzielas and S.~F.~King,
  %``Towards a complete $\Delta(27) \times SO(10)$ SUSY GUT,''
  Phys.\ Rev.\ D {\bf 94} (2016) no.1,  016006
  doi:10.1103/PhysRevD.94.016006
  [arXiv:1512.00850 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.016006;%%
  %24 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Vien:2016tmh}
\bibitem{Vien:2016tmh}
  V.~V.~Vien, A.~E.~Cárcamo Hernández and H.~N.~Long,
  %``The $\Delta(27)$ flavor 3-3-1 model with neutral leptons,''
  Nucl.\ Phys.\ B {\bf 913} (2016) 792
  doi:10.1016/j.nuclphysb.2016.10.010
  [arXiv:1601.03300 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2016.10.010;%%
  %24 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Hernandez:2016eod}
\bibitem{Hernandez:2016eod}
  A.~E.~Cárcamo Hernández, H.~N.~Long and V.~V.~Vien,
  %``A 3-3-1 model with right-handed neutrinos based on the $\varDelta \left( 27\right) $ family symmetry,''
  Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.5,  242
  doi:10.1140/epjc/s10052-016-4074-0
  [arXiv:1601.05062 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-4074-0;%%
  %19 citations counted in INSPIRE as of 12 Mar 2018



%\cite{CarcamoHernandez:2017owh}
\bibitem{CarcamoHernandez:2017owh}
  A.~E.~Cárcamo Hernández, S.~Kovalenko, J.~W.~F.~Valle and C.~A.~Vaquera-Araujo,
  %``Predictive Pati-Salam theory of fermion masses and mixing,''
  JHEP {\bf 1707} (2017) 118
  doi:10.1007/JHEP07(2017)118
  [arXiv:1705.06320 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2017)118;%%
  %9 citations counted in INSPIRE as of 12 Mar 2018



%\cite{deMedeirosVarzielas:2017sdv}
\bibitem{deMedeirosVarzielas:2017sdv}
  I.~de Medeiros Varzielas, G.~G.~Ross and J.~Talbert,
  %``A Unified Model of Quarks and Leptons with a Universal Texture Zero,''
  JHEP {\bf 1803} (2018) 007
  doi:10.1007/JHEP03(2018)007
  [arXiv:1710.01741 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2018)007;%%
  %3 citations counted in INSPIRE as of 12 Mar 2018



%\cite{CarcamoHernandez:2018iel}
\bibitem{CarcamoHernandez:2018iel}
  A.~E.~Cárcamo Hernández, H.~N.~Long and V.~V.~Vien,
  %``Fermion masses and mixings in a 3-3-1 model with $\Delta\left(27\right)$ family symmetry and inverse seesaw mechanism,''
  arXiv:1803.01636 [hep-ph].
  %%CITATION = ARXIV:1803.01636;%%



%\cite{Ade:2015xua}
\bibitem{Ade:2015xua}
  P.~A.~R.~Ade {\it et al.} [Planck Collaboration],
  %``Planck 2015 results. XIII. Cosmological parameters,''
  Astron.\ Astrophys.\  {\bf 594} (2016) A13
  doi:10.1051/0004-6361/201525830
  [arXiv:1502.01589 [astro-ph.CO]].
  %%CITATION = doi:10.1051/0004-6361/201525830;%%
  %5166 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bergstrom:2000pn}
\bibitem{Bergstrom:2000pn}
  L.~Bergström,
  %``Nonbaryonic dark matter: Observational evidence and detection methods,''
  Rept.\ Prog.\ Phys.\  {\bf 63} (2000) 793
  doi:10.1088/0034-4885/63/5/2r3
  [hep-ph/0002126].
  %%CITATION = doi:10.1088/0034-4885/63/5/2r3;%%
  %668 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bertone:2016nfn}
\bibitem{Bertone:2016nfn}
  G.~Bertone and D.~Hooper,
  %``A History of Dark Matter,''
  %Submitted to: Rev.Mod.Phys.
  [arXiv:1605.04909 [astro-ph.CO]].
  %%CITATION = ARXIV:1605.04909;%%
  %72 citations counted in INSPIRE as of 12 Mar 2018



%\cite{deSwart:2017heh}
\bibitem{deSwart:2017heh}
  J.~de Swart, G.~Bertone and J.~van Dongen,
  %``How Dark Matter Came to Matter,''
  Nature Astron.\  {\bf 1} (2017) 0059
  doi:10.1038/s41550017-0059, 10.1038/s41550-017-0059
  [arXiv:1703.00013 [astro-ph.CO]].
  %%CITATION = doi:10.1038/s41550017-0059, 10.1038/s41550-017-0059;%%
  %12 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Arcadi:2017kky}
\bibitem{Arcadi:2017kky}
  G.~Arcadi, M.~Dutra, P.~Ghosh, M.~Lindner, Y.~Mambrini, M.~Pierre, S.~Profumo and F.~S.~Queiroz,
  %``The waning of the WIMP? A review of models, searches, and constraints,''
  Eur.\ Phys.\ J.\ C {\bf 78} (2018) no.3,  203
  doi:10.1140/epjc/s10052-018-5662-y
  [arXiv:1703.07364 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-018-5662-y;%%
  %78 citations counted in INSPIRE as of 12 Mar 2018



%\cite{McDonald:2001vt}
\bibitem{McDonald:2001vt}
  J.~McDonald,
  %``Thermally generated gauge singlet scalars as selfinteracting dark matter,''
  Phys.\ Rev.\ Lett.\  {\bf 88} (2002) 091304
  doi:10.1103/PhysRevLett.88.091304
  [hep-ph/0106249].
  %%CITATION = doi:10.1103/PhysRevLett.88.091304;%%
  %170 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Choi:2005vq}
\bibitem{Choi:2005vq}
  K.~Y.~Choi and L.~Roszkowski,
  %``E-WIMPs,''
  AIP Conf.\ Proc.\  {\bf 805} (2006) 30
  doi:10.1063/1.2149672
  [hep-ph/0511003].
  %%CITATION = doi:10.1063/1.2149672;%%
  %27 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Kusenko:2006rh}
\bibitem{Kusenko:2006rh}
  A.~Kusenko,
  %``Sterile neutrinos, dark matter, and the pulsar velocities in models with a Higgs singlet,''
  Phys.\ Rev.\ Lett.\  {\bf 97} (2006) 241301
  doi:10.1103/PhysRevLett.97.241301
  [hep-ph/0609081].
  %%CITATION = doi:10.1103/PhysRevLett.97.241301;%%
  %217 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Hall:2009bx}
\bibitem{Hall:2009bx}
  L.~J.~Hall, K.~Jedamzik, J.~March-Russell and S.~M.~West,
  %``Freeze-In Production of FIMP Dark Matter,''
  JHEP {\bf 1003} (2010) 080
  doi:10.1007/JHEP03(2010)080
  [arXiv:0911.1120 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2010)080;%%
  %283 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Petraki:2007gq}
\bibitem{Petraki:2007gq}
  K.~Petraki and A.~Kusenko,
  %``Dark-matter sterile neutrinos in models with a gauge singlet in the Higgs sector,''
  Phys.\ Rev.\ D {\bf 77} (2008) 065014
  doi:10.1103/PhysRevD.77.065014
  [arXiv:0711.4646 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.065014;%%
  %180 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bernal:2017kxu}
\bibitem{Bernal:2017kxu}
  N.~Bernal, M.~Heikinheimo, T.~Tenkanen, K.~Tuominen and V.~Vaskonen,
  %``The Dawn of FIMP Dark Matter: A Review of Models and Constraints,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 32} (2017) no.27,  1730023
  doi:10.1142/S0217751X1730023X
  [arXiv:1706.07442 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X1730023X;%%
  %32 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Ma:2006km}
\bibitem{Ma:2006km}
  E.~Ma,
  %``Verifiable radiative seesaw mechanism of neutrino mass and dark matter,''
  Phys.\ Rev.\ D {\bf 73} (2006) 077301
  doi:10.1103/PhysRevD.73.077301
  [hep-ph/0601225].
  %%CITATION = doi:10.1103/PhysRevD.73.077301;%%
  %768 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Hernandez:2013dta}
\bibitem{Hernandez:2013dta}
  A.~E.~Carcamo Hernandez, I.~de Medeiros Varzielas, S.~G.~Kovalenko, H.~Päs and I.~Schmidt,
  %``Lepton masses and mixings in an $A_4$ multi-Higgs model with a radiative seesaw mechanism,''
  Phys.\ Rev.\ D {\bf 88} (2013) no.7,  076014
  doi:10.1103/PhysRevD.88.076014
  [arXiv:1307.6499 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.076014;%%
  %60 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Campos:2014lla}
\bibitem{Campos:2014lla}
  M.~D.~Campos, A.~E.~Cárcamo Hernández, S.~Kovalenko, I.~Schmidt and E.~Schumacher,
  %``Fermion masses and mixings in an $SU(5)$ grand unified model with an extra flavor symmetry,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.1,  016006
  doi:10.1103/PhysRevD.90.016006
  [arXiv:1403.2525 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.016006;%%
  %28 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Hernandez:2015hrt}
\bibitem{Hernandez:2015hrt}
  A.~E.~Cárcamo Hernández,
  %``A novel and economical explanation for SM fermion masses and mixings,''
  Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.9,  503
  doi:10.1140/epjc/s10052-016-4351-y
  [arXiv:1512.09092 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-4351-y;%%
  %85 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2015joa}
\bibitem{Varzielas:2015joa}
  I.~de Medeiros Varzielas, O.~Fischer and V.~Maurer,
  %``$ {\mathbb{A}}_4 $ symmetry at colliders and in the universe,''
  JHEP {\bf 1508} (2015) 080
  doi:10.1007/JHEP08(2015)080
  [arXiv:1504.03955 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2015)080;%%
  %44 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Arbelaez:2016mhg}
\bibitem{Arbelaez:2016mhg}
  C.~Arbeláez, A.~E.~Cárcamo Hernández, S.~Kovalenko and I.~Schmidt,
  %``Radiative Seesaw-type Mechanism of Fermion Masses and Non-trivial Quark Mixing,''
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.6,  422
  doi:10.1140/epjc/s10052-017-4948-9
  [arXiv:1602.03607 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-4948-9;%%
  %42 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Kownacki:2016hpm}
\bibitem{Kownacki:2016hpm}
  C.~Kownacki and E.~Ma,
  %``Gauge $U(1)$ dark symmetry and radiative light fermion masses,''
  Phys.\ Lett.\ B {\bf 760} (2016) 59
  doi:10.1016/j.physletb.2016.06.024
  [arXiv:1604.01148 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2016.06.024;%%
  %21 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Nomura:2016emz}
\bibitem{Nomura:2016emz}
  T.~Nomura and H.~Okada,
  %``Radiatively induced Quark and Lepton Mass Model,''
  Phys.\ Lett.\ B {\bf 761} (2016) 190
  doi:10.1016/j.physletb.2016.08.023
  [arXiv:1606.09055 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2016.08.023;%%
  %19 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Nomura:2016pgg}
\bibitem{Nomura:2016pgg}
  T.~Nomura and H.~Okada,
  %``Two-loop Induced Majorana Neutrino Mass in a Radiatively Induced Quark and Lepton Mass Model,''
  Phys.\ Rev.\ D {\bf 94} (2016) no.9,  093006
  doi:10.1103/PhysRevD.94.093006
  [arXiv:1609.01504 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.093006;%%
  %15 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Nomura:2016dnf}
\bibitem{Nomura:2016dnf}
  T.~Nomura, H.~Okada and Y.~Orikasa,
  %``Radiative neutrino model with $SU(2)_L$ triplet fields,''
  Phys.\ Rev.\ D {\bf 94} (2016) no.11,  115018
  doi:10.1103/PhysRevD.94.115018
  [arXiv:1610.04729 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.115018;%%
  %10 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Chulia:2016ngi}
\bibitem{Chulia:2016ngi}
  S.~Centelles Chuliá, E.~Ma, R.~Srivastava and J.~W.~F.~Valle,
  %``Dirac Neutrinos and Dark Matter Stability from Lepton Quarticity,''
  Phys.\ Lett.\ B {\bf 767} (2017) 209
  doi:10.1016/j.physletb.2017.01.070
  [arXiv:1606.04543 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2017.01.070;%%
  %22 citations counted in INSPIRE as of 12 Mar 2018



%\cite{CarcamoHernandez:2016pdu}
\bibitem{CarcamoHernandez:2016pdu}
  A.~E.~Cárcamo Hernández, S.~Kovalenko and I.~Schmidt,
  %``Radiatively generated hierarchy of lepton and quark masses,''
  JHEP {\bf 1702} (2017) 125
  doi:10.1007/JHEP02(2017)125
  [arXiv:1611.09797 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2017)125;%%
  %7 citations counted in INSPIRE as of 12 Mar 2018



%\cite{CarcamoHernandez:2017kra}
\bibitem{CarcamoHernandez:2017kra}
  A.~E.~Cárcamo Hernández and H.~N.~Long,
  %``A highly predictive $A_{4}$ flavour 3-3-1 model with radiative inverse seesaw mechanism,''
  arXiv:1705.05246 [hep-ph].
  %%CITATION = ARXIV:1705.05246;%%
  %6 citations counted in INSPIRE as of 12 Mar 2018



%\cite{CarcamoHernandez:2017cwi}
\bibitem{CarcamoHernandez:2017cwi}
  A.~E.~Cárcamo Hernández, S.~Kovalenko, H.~N.~Long and I.~Schmidt,
  %``A variant of 3-3-1 model for the generation of the SM fermion mass and mixing pattern,''
  arXiv:1705.09169 [hep-ph].
  %%CITATION = ARXIV:1705.09169;%%
  %4 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Alvarado:2017bax}
\bibitem{Alvarado:2017bax}
  C.~Alvarado, F.~Elahi and N.~Raj,
  %``Thermal dark matter via the flavon portal,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.7,  075002
  doi:10.1103/PhysRevD.96.075002
  [arXiv:1706.03081 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.075002;%%



%\cite{Calibbi:2015sfa}
\bibitem{Calibbi:2015sfa}
  L.~Calibbi, A.~Crivellin and B.~Zaldívar,
  %``Flavor portal to dark matter,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.1,  016004
  doi:10.1103/PhysRevD.92.016004
  [arXiv:1501.07268 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.016004;%%
  %26 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Varzielas:2015sno}
\bibitem{Varzielas:2015sno}
  I.~de Medeiros Varzielas and O.~Fischer,
  %``Non-Abelian family symmetries as portals to dark matter,''
  JHEP {\bf 1601} (2016) 160
  doi:10.1007/JHEP01(2016)160
  [arXiv:1512.00869 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2016)160;%%
  %11 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Hernandez:2014zsa}
\bibitem{Hernandez:2014zsa}
  A.~E.~Cárcamo Hernández and I.~de Medeiros Varzielas,
  %``Viable textures for the fermion sector,''
  J.\ Phys.\ G {\bf 42} (2015) no.6,  065002
  doi:10.1088/0954-3899/42/6/065002
  [arXiv:1410.2481 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/42/6/065002;%%
  %19 citations counted in INSPIRE as of 12 Mar 2018



%\cite{deMedeirosVarzielas:2017glw}
\bibitem{deMedeirosVarzielas:2017glw}
  I.~de Medeiros Varzielas, S.~F.~King, C.~Luhn and T.~Neder,
  %``Minima of multi-Higgs potentials with triplets of $\Delta(3n^2)$ and $\Delta(6n^2)$,''
  Phys.\ Lett.\ B {\bf 775} (2017) 303
  doi:10.1016/j.physletb.2017.11.005
  [arXiv:1704.06322 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2017.11.005;%%
  %4 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bora:2012tx}
\bibitem{Bora:2012tx}
  K.~Bora,
  %``Updated values of running quark and lepton masses at GUT scale in SM, 2HDM and MSSM,''
  Horizon {\bf 2} (2013)
  [arXiv:1206.5909 [hep-ph]].
  %%CITATION = ARXIV:1206.5909;%%
  %31 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Xing:2007fb}
\bibitem{Xing:2007fb}
  Z.~z.~Xing, H.~Zhang and S.~Zhou,
  %``Updated Values of Running Quark and Lepton Masses,''
  Phys.\ Rev.\ D {\bf 77} (2008) 113016
  doi:10.1103/PhysRevD.77.113016
  [arXiv:0712.1419 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.113016;%%
  %314 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Olive:2016xmw}
\bibitem{Olive:2016xmw}
  C.~Patrignani {\it et al.} [Particle Data Group],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 40} (2016) no.10,  100001.
  doi:10.1088/1674-1137/40/10/100001
  %%CITATION = doi:10.1088/1674-1137/40/10/100001;%%
  %2776 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Agashe:2014kda}
\bibitem{Agashe:2014kda}
  K.~A.~Olive {\it et al.} [Particle Data Group],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 38} (2014) 090001.
  doi:10.1088/1674-1137/38/9/090001
  %%CITATION = doi:10.1088/1674-1137/38/9/090001;%%
  %7111 citations counted in INSPIRE as of 12 Mar 2018



%\cite{deSalas:2017kay}
\bibitem{deSalas:2017kay}
  P.~F.~de Salas, D.~V.~Forero, C.~A.~Ternes, M.~Tortola and J.~W.~F.~Valle,
  %``Status of neutrino oscillations 2017,''
  arXiv:1708.01186 [hep-ph].
  %%CITATION = ARXIV:1708.01186;%%
  %69 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Alessandria:2011rc}
\bibitem{Alessandria:2011rc}
  F.~Alessandria {\it et al.} [CUORE Collaboration],
  %``Sensitivity of CUORE to Neutrinoless Double-Beta Decay,''
  arXiv:1109.0494 [nucl-ex].
  %%CITATION = ARXIV:1109.0494;%%
  %82 citations counted in INSPIRE as of 12 Mar 2018



%\cite{KamLAND-Zen:2016pfg}
\bibitem{KamLAND-Zen:2016pfg}
  A.~Gando {\it et al.} [KamLAND-Zen Collaboration],
  %``Search for Majorana Neutrinos near the Inverted Mass Hierarchy Region with KamLAND-Zen,''
  Phys.\ Rev.\ Lett.\  {\bf 117} (2016) no.8,  082503
   Addendum: [Phys.\ Rev.\ Lett.\  {\bf 117} (2016) no.10,  109903]
  doi:10.1103/PhysRevLett.117.109903, 10.1103/PhysRevLett.117.082503
  [arXiv:1605.02889 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.117.109903, 10.1103/PhysRevLett.117.082503;%%
  %234 citations counted in INSPIRE as of 12 Mar 2018


%\cite{Varzielas:2010mp}
\bibitem{Varzielas:2010mp}
  I.~de Medeiros Varzielas and L.~Merlo,
  %``Ultraviolet Completion of Flavour Models,''
  JHEP {\bf 1102} (2011) 062
  doi:10.1007/JHEP02(2011)062
  [arXiv:1011.6662 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2011)062;%%
  %44 citations counted in INSPIRE as of 28 Sep 2016



%\cite{Belanger:2006is}
\bibitem{Belanger:2006is}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``MicrOMEGAs 2.0: A Program to calculate the relic density of dark matter in a generic model,''
  Comput.\ Phys.\ Commun.\  {\bf 176} (2007) 367
  doi:10.1016/j.cpc.2006.11.008
  [hep-ph/0607059].
  %%CITATION = doi:10.1016/j.cpc.2006.11.008;%%
  %587 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Belanger:2008sj}
\bibitem{Belanger:2008sj}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``Dark matter direct detection rate in a generic model with micrOMEGAs 2.2,''
  Comput.\ Phys.\ Commun.\  {\bf 180} (2009) 747
  doi:10.1016/j.cpc.2008.11.019
  [arXiv:0803.2360 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2008.11.019;%%
  %565 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Belanger:2010pz}
\bibitem{Belanger:2010pz}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``micrOMEGAs: A Tool for dark matter studies,''
  Nuovo Cim.\ C {\bf 033N2} (2010) 111
  doi:10.1393/ncc/i2010-10591-3
  [arXiv:1005.4133 [hep-ph]].
  %%CITATION = doi:10.1393/ncc/i2010-10591-3;%%
  %85 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Belanger:2013oya}
\bibitem{Belanger:2013oya}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``micrOMEGAs3: A program for calculating dark matter observables,''
  Comput.\ Phys.\ Commun.\  {\bf 185} (2014) 960
  doi:10.1016/j.cpc.2013.10.016
  [arXiv:1305.0237 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2013.10.016;%%
  %467 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Cui:2017nnn}
\bibitem{Cui:2017nnn}
  X.~Cui {\it et al.} [PandaX-II Collaboration],
  %``Dark Matter Results From 54-Ton-Day Exposure of PandaX-II Experiment,''
  Phys.\ Rev.\ Lett.\  {\bf 119} (2017) no.18,  181302
  doi:10.1103/PhysRevLett.119.181302
  [arXiv:1708.06917 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevLett.119.181302;%%
  %118 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Green:2002ht}
\bibitem{Green:2002ht}
  A.~M.~Green,
  %``Effect of halo modeling on WIMP exclusion limits,''
  Phys.\ Rev.\ D {\bf 66} (2002) 083003
  doi:10.1103/PhysRevD.66.083003
  [astro-ph/0207366].
  %%CITATION = doi:10.1103/PhysRevD.66.083003;%%
  %84 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Zemp:2008gw}
\bibitem{Zemp:2008gw}
  M.~Zemp, J.~Diemand, M.~Kuhlen, P.~Madau, B.~Moore, D.~Potter, J.~Stadel and L.~Widrow,
  %``The Graininess of Dark Matter Haloes,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 394} (2009) 641
  doi:10.1111/j.1365-2966.2008.14361.x
  [arXiv:0812.2033 [astro-ph]].
  %%CITATION = doi:10.1111/j.1365-2966.2008.14361.x;%%
  %63 citations counted in INSPIRE as of 12 Mar 2018



%\cite{McCabe:2010zh}
\bibitem{McCabe:2010zh}
  C.~McCabe,
  %``The Astrophysical Uncertainties Of Dark Matter Direct Detection Experiments,''
  Phys.\ Rev.\ D {\bf 82} (2010) 023530
  doi:10.1103/PhysRevD.82.023530
  [arXiv:1005.0579 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.82.023530;%%
  %140 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Pato:2010yq}
\bibitem{Pato:2010yq}
  M.~Pato, O.~Agertz, G.~Bertone, B.~Moore and R.~Teyssier,
  %``Systematic uncertainties in the determination of the local dark matter density,''
  Phys.\ Rev.\ D {\bf 82} (2010) 023531
  doi:10.1103/PhysRevD.82.023531
  [arXiv:1006.1322 [astro-ph.HE]].
  %%CITATION = doi:10.1103/PhysRevD.82.023531;%%
  %103 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Fairbairn:2012zs}
\bibitem{Fairbairn:2012zs}
  M.~Fairbairn, T.~Douce and J.~Swift,
  %``Quantifying Astrophysical Uncertainties on Dark Matter Direct Detection Results,''
  Astropart.\ Phys.\  {\bf 47} (2013) 45
  doi:10.1016/j.astropartphys.2013.06.003
  [arXiv:1206.2693 [astro-ph.CO]].
  %%CITATION = doi:10.1016/j.astropartphys.2013.06.003;%%
  %40 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bernal:2014mmt}
\bibitem{Bernal:2014mmt}
  N.~Bernal, J.~E.~Forero-Romero, R.~Garani and S.~Palomares-Ruiz,
  %``Systematic uncertainties from halo asphericity in dark matter searches,''
  JCAP {\bf 1409} (2014) 004
  doi:10.1088/1475-7516/2014/09/004
  [arXiv:1405.6240 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2014/09/004;%%
  %22 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bernal:2015oyn}
\bibitem{Bernal:2015oyn}
  N.~Bernal, J.~E.~Forero-Romero, R.~Garani and S.~Palomares-Ruiz,
  %``Systematic uncertainties from halo asphericity in dark matter searches,''
  Nucl.\ Part.\ Phys.\ Proc.\  {\bf 267-269} (2015) 345.
  doi:10.1016/j.nuclphysbps.2015.10.129
  %%CITATION = doi:10.1016/j.nuclphysbps.2015.10.129;%%
  %3 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Bernal:2016guq}
\bibitem{Bernal:2016guq}
  N.~Bernal, L.~Necib and T.~R.~Slatyer,
  %``Spherical Cows in Dark Matter Indirect Detection,''
  JCAP {\bf 1612} (2016) no.12,  030
  doi:10.1088/1475-7516/2016/12/030
  [arXiv:1606.00433 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2016/12/030;%%
  %7 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Benito:2016kyp}
\bibitem{Benito:2016kyp}
  M.~Benito, N.~Bernal, N.~Bozorgnia, F.~Calore and F.~Iocco,
  %``Particle Dark Matter Constraints: the Effect of Galactic Uncertainties,''
  JCAP {\bf 1702} (2017) no.02,  007
  doi:10.1088/1475-7516/2017/02/007
  [arXiv:1612.02010 [hep-ph]].
  %%CITATION = doi:10.1088/1475-7516/2017/02/007;%%
  %13 citations counted in INSPIRE as of 12 Mar 2018



%\cite{Green:2017odb}
\bibitem{Green:2017odb}
  A.~M.~Green,
  %``Astrophysical uncertainties on the local dark matter distribution and direct detection experiments,''
  J.\ Phys.\ G {\bf 44} (2017) no.8,  084001
  doi:10.1088/1361-6471/aa7819
  [arXiv:1703.10102 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1361-6471/aa7819;%%
  %13 citations counted in INSPIRE as of 12 Mar 2018


\bibitem{Farina:2009ez} 
  M.~Farina, D.~Pappadopulo and A.~Strumia,
  %``CDMS stands for Constrained Dark Matter Singlet,''
  Phys.\ Lett.\ B {\bf 688}, 329 (2010)
  doi:10.1016/j.physletb.2010.04.025
  [arXiv:0912.5038 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2010.04.025;%%
  %60 citations counted in INSPIRE as of 22 Mar 2018

\bibitem{Giedt:2009mr} 
  J.~Giedt, A.~W.~Thomas and R.~D.~Young,
  %``Dark matter, the CMSSM and lattice QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 103}, 201802 (2009)
  doi:10.1103/PhysRevLett.103.201802
  [arXiv:0907.4177 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.103.201802;%%
  %185 citations counted in INSPIRE as of 22 Mar 2018


